FlexiNS: A SmartNIC-Centric, Line-Rate and Flexible Network Stack

As the gap between network and CPU speeds rapidly increases, the CPU-centric network stack proves inadequate due to excessive CPU and memory overhead. While hardware-offloaded network stacks alleviate these issues, they suffer from limited flexibility in both control and data planes. Offloading network stack to off-path SmartNIC seems promising to provide high flexibility; however, throughput remains constrained by inherent SmartNIC architectural limitations. To this end, we design FlexiNS, a SmartNIC-centric network stack with software transport programmability and line-rate packet processing capabilities. To grapple with the limitation of SmartNIC-induced challenges, FlexiNS introduces: (a) a header-only offloading TX path; (b) an unlimited-working-set in-cache processing RX path; (c) a high-performance DMA-only notification pipe; and (d) a programmable offloading engine. We prototype FlexiNS using Nvidia BlueField-3 SmartNIC and provide out-of-the-box RDMA IBV verbs compatibility to users. FlexiNS achieves 2.2$\times$ higher throughput than the microkernel-based baseline in block storage disaggregation and 1.3$\times$ higher throughput than the hardware-offloaded baseline in KVCache transfer.

==> content/3-background.tex <==
\section{BACKGROUND}
